Step-by-step Layered Design Generation

Design generation, in its essence, is a step-by-step process where designers progressively refine and enhance their work through careful modifications. Despite this fundamental characteristic, existing approaches mainly treat design synthesis as a single-step generation problem, significantly underestimating the inherent complexity of the creative process. To bridge this gap, we propose a novel problem setting called Step-by-Step Layered Design Generation, which tasks a machine learning model with generating a design that adheres to a sequence of instructions from a designer. Leveraging recent advancements in multi-modal LLMs, we propose SLEDGE: Step-by-step LayEred Design GEnerator to model each update to a design as an atomic, layered change over its previous state, while being grounded in the instruction. To complement our new problem setting, we introduce a new evaluation suite, including a dataset and a benchmark. Our exhaustive experimental analysis and comparison with state-of-the-art approaches tailored to our new setup demonstrate the efficacy of our approach. We hope our work will attract attention to this pragmatic and under-explored research area.

==> CameraReady/figs/data_samples.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.48\textwidth]{figs/images/data_samples.pdf}
  \caption{Qualitative examples from our dataset illustrating the complex edits involved in the design generation task. }
  \label{fig:data_samples}
\end{figure}

==> CameraReady/figs/human.tex <==
\pgfplotsset{compat=1.17}
\begin{tikzpicture}
\begin{axis}[
    ybar stacked,  % This makes the bars stack
    bar width=15pt,
    width=6cm, 
    height=4.5cm,
    xlabel={},
    ylabel={Percentage},
    title={Human Evaluation},
    symbolic x coords={Theme Ad., Aesthetic Q., Edit Comp.},
    xtick=data,
    legend style={at={(0.5,-0.2)}, 
                  anchor=north, 
                  legend columns=2},
    ymin=0,
    nodes near coords,
    nodes near coords align={vertical}
]

% Bottom portion of each bar
\addplot[fill=yellow!70, draw=black] coordinates {
    (Theme Ad., 37)
    (Aesthetic Q., 41)
    (Edit Comp., 37.5)
};

% Top portion of each bar
\addplot[fill=red!70, draw=black] coordinates {
    (Theme Ad., 63)
    (Aesthetic Q., 59)
    (Edit Comp., 62.5)
};

\legend{Baselines, Ours}
\end{axis}
\end{tikzpicture}

==> CameraReady/sec/0_abstract.tex <==
\begin{abstract}
Design generation, in its essence, is a step-by-step process where designers progressively refine and enhance their work through careful modifications. Despite this fundamental characteristic, existing approaches mainly treat design synthesis as a single-step generation problem, significantly underestimating the inherent complexity of the creative process. 
To bridge this gap, we propose a novel problem setting called Step-by-step Layered Design Generation, that tasks a machine learning model to generate a design, adhering to a sequence of instructions from a designer. 
Leveraging the recent advancements in multi-modal LLMs, we propose SLEDGE: Step-by-step LayEred Design GEnerator to model each update to a design as an atomic layered change over its previous state, while being grounded on the instruction.
To complement our new problem setting, we introduce a new evaluation suite, including a dataset and a benchmark. Our exhaustive experimental analysis and comparison with state-of-the-art approaches adapted to our new setup bring out the efficacy of our approach. 
We hope our work will attract attention to this pragmatic and under-explored research area.
\end{abstract}

==> CameraReady/tables/ablations.tex <==
\resizebox{\columnwidth}{!}{
\begin{tabular}{lrrr}
\midrule
& Variant & Both & \ourmethod \\
\midrule
w/o$~\mathcal{D}$ Finetune & 27.0\% & 32.0\% & 41.0\% \\
Local Loss & 22.7\% & 52.2\% & 25.1\% \\
$\mathcal{U_{\text{t+1}}}$ Empty & 26.0\% & 44.0\% & 30.0\% \\
\midrule
\end{tabular}
\label{tab:ablation}
}

==> CameraReady/tables/human_eval.tex <==
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrr|rlr|rlr}
\midrule
& \multicolumn{3}{c}{ZONE} & \multicolumn{3}{c}{Ranni} & \multicolumn{3}{c}{LLMGA} \\
& ZONE~\cite{zone} & Both & Ours & Ranni~\cite{ranni} & Both & Ours &LLMGA~\cite{llmga} & Both & Ours \\
\midrule
Theme & 1.0\% & 4.4\% & 94.6\% & 1.0\% & 7.5\% & 91.7\% & 25.9\% & 44.1\% & 30.0\%\\
Edit & 3.0\% & 8.2\% & 88.8\% & 2.1\% & 9.7\% & 88.2\% & 13\% & 33\% & 54\%\\
Final & 1.2\% & 6.9\% & 94.6\% & 1.0\% & 12.0\% & 87.0\% & 23.0\% & 41.9\% & 35.1\% \\
\midrule
\end{tabular}
\label{tab:baselines}
}


==> CameraReady/tables/intern_comp.tex <==

\resizebox{\textwidth}{!}{
\begin{tabular}{lrrr|rlr|rlr}
\midrule
& ZONE~\cite{zone} & Both & Ours & Ranni~\cite{ranni} & Both & Ours &T2I+LLMGA~\cite{llmga} & Both & Ours \\
\midrule
Theme Adherence & 1.0\% & 4.4\% & 94.6\% & 1.0\% & 7.5\% & 91.7\% & 25.9\% & 44.1\% & 30.0\%\\
Aesthetics Quality & 1.2\% & 6.9\% & 94.6\% & 1.0\% & 12.0\% & 87.0\% & 23.0\% & 41.9\% & 35.1\% \\
Edit Compliance & 3.0\% & 8.2\% & 88.8\% & 2.1\% & 9.7\% & 88.2\% & 13\% & 33\% & 54\%\\
\midrule
\end{tabular}
\label{tab:baselines}
}
